Review of lattice results concerning low energy particle physics

We review lattice results relevant for pion and kaon physics with the aim of making them easily accessible to the particle physics community. Specifically, we review the determination of the light-quark masses, the form factor f_+(0), relevant for the semileptonic K -> pi transition at zero momentum transfer as well as the ratio f_K/f_pi of decay constants and discuss the consequences for the elements V_{us} and V_{ud} of the CKM matrix. Furthermore, we describe the results obtained on the lattice for some of the low-energy constants of SU(2)_LxSU(2)_R and SU(3)_LxSU(3)_R Chiral Perturbation Theory and review the determination of the B_K parameter of neutral kaon mixing. We introduce quality criteria and use these when forming averages. Although subjective and imperfect, these criteria may help the reader to judge different aspects of current lattice computations. Our main results are summarized in section 1.2, but we stress the importance of the detailed discussion that underlies these results and constitutes the bulk of the present review.

==> app.tex <==

\subsection{Notes to section \ref{sec_MF}}


\bigskip
\bigskip
\par\noindent
{\bf Continuum extrapolations/estimation of lattice artifacts:}\\
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c l l}
&&&& \\[-0.1cm]
\hline\hline
&&&& \\[-0.3cm]
Collab. & Ref. & $\Nf$ & $a$[fm]& Description \\
\hline\hline
&&&& \\[-0.1cm]
%
CERN-TOV 07 & \cite{DelDebbio:2006cn} & 2 & 0.0717(15),0.0521(7)& Scale fixed through $M_K$.\\
            &                         &   & 0.0784(10)          & Non-perturbatively $O(a)$ impr. \\
[3.0ex] \hline \\[-1.0ex]
%
ETMC 07,08A & \cite{Blossier:2007vv,Dimopoulos:2008sy}  & 2 & 0.0855(5),0.0667(5) & \parbox{7cm}{Automatic $O(a)$ impr., flavour symmetry
  breaking: $(M_{PS}^{0})^2-(M_{PS}^\pm)^2\sim O(a^2)$. \\
  Scale fixed through $F_\pi$.}\\
            &                                &   & 0.1             &            not included in extrapolation.\\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 08A & \cite{Noaki:2008iy} & 2 & 0.1184(3)(21)
& \parbox{7cm}{Automatic $O(a)$ impr., exact chiral symmetry. Scale fixed through $r_0$.}\\
[3.0ex] \hline \\[-1.0ex]
%
RBC/UKQCD 08 & \cite{Allton:2008pn} & 2 &  0.1141(18)
& \parbox{7cm}{Fifth dimension with extension $L_s$; exact chiral
  symmetry and $O(a)$ improvement in the limit $L_s\rightarrow
  \infty$. Scale fixed through $\Omega$ baryon mass. Add 4$\%$ systematic error for lattice artifacts.}\\
[3.0ex] \hline \\[-1.0ex]
%
PACS-CS 08 & \cite{Aoki:2008sm} & 2 & 0.0907(13)
& \parbox{7cm}{Non-perturbatively $O(a)$ improved. Scale fixed through
  the $\Omega$ baryon mass. }\\
[3.0ex] \hline \\[-1.0ex]
%
HHS 08 & \cite{Hasenfratz:2008ce} & 2 & 0.1153(5) & tree level $O(a)$
improvement. Scale fixed through $r_0$.\\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 07B & \cite{Fukaya:2007pn} & 2 & 0.1111(24) & \parbox{7cm}{Automatic $O(a)$ impr., exact chiral symmetry. Scale fixed through $r_0$.} \\
\hline\hline
%
\end{tabular*}
}



\newpage


\bigskip
\bigskip
\par\noindent
{\bf Chiral extrapolation/minimum pion mass:}\\
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c l}
&&&& \\[-0.1cm]
\hline\hline
&&&& \\[-0.3cm]
Collab. & Ref. & $\Nf$ & $M_{\pi,\text{min}}$ [MeV] & Description \\
\hline\hline
&&&& \\[-0.1cm]
%
CERN-TOV 07 & \cite{DelDebbio:2006cn} & 2 & 403, 381, 377 & \parbox{6cm}{NLO SU(2) fit up to $M_\pi\simeq $ 540 MeV.}\\
[3.0ex] \hline \\[-1.0ex]
%
ETMC 07,08A & \cite{Blossier:2007vv,Dimopoulos:2008sy} & 2 & 265, 300 & \parbox{6cm}{NLO SU(2) fit. NNLO fit to estimate systematic error.} \\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 08A & \cite{Noaki:2008iy} & 2 & 290 & \parbox{6cm}{NNLO SU(2) fit up to $M_\pi=$ 750 MeV.}\\
[3.0ex] \hline \\[-1.0ex]
%
RBC/UKQCD 08 & \cite{Allton:2008pn} & 2 & 330 & \parbox{6cm}{Partially quenched SU(2) fit at NLO. Interpolation to the physical $m_s$.} \\
[3.0ex] \hline \\[-1.0ex]
%
PACS-CS 08 & \cite{Aoki:2008sm} & 2 & 160 & \parbox{6cm}{SU(2) fit at
  NLO, only unitary points. Linear expansion around physical $m_s$.}\\
[3.0ex] \hline \\[-1.0ex]
%
HHS 08 & \cite{Hasenfratz:2008ce} & 2 &  \parbox{3.5cm}{$\mu_{\rm min}=m\Sigma
V_1\simeq 0.7-2.9$\\ $\mu=m\Sigma V_2\simeq 2.1-5.0$}
&  \parbox{6cm}{$\epsilon$-regime: higher values might be too large to
  be considered in the $\epsilon$-regime.  NLO SU(2) $\epsilon$-regime fit.}\\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 07B & \cite{Fukaya:2007pn} & 2 & $\mu=m\Sigma V\simeq 0.556$ & \parbox{5cm}{NLO SU(2) $\epsilon$-regime fit.} \\
[3.0ex]
\hline\hline
%
\end{tabular*}
}



\bigskip
\bigskip
\par\noindent
{\bf Finite volume effects:}\\
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c c c l}
&&&&& \\[-0.1cm]
\hline\hline
&&&&& \\[-0.3cm]
Collab. & Ref. & $\Nf$ & $L$ [fm] & $M_{\pi,\text{min}} L$ & Description \\
\hline\hline
&&&&& \\[-0.1cm]
%
CERN-TOV 07 & \cite{DelDebbio:2006cn} & 2 & 1.72, 1.67, 1.88 & 3.5, 3.2, 3.6 & \\
[3.0ex] \hline \\[-1.0ex]
%
ETMC 07,08A & \cite{Blossier:2007vv,Dimopoulos:2008sy} & 2 & \parbox{2.5cm}{2.05, 2.74, 1.33,
1.60, 2.13} & 3.7, 3.2 & \parbox{5cm}{Finite-volume effects estimated through \protect\cite{Colangelo:2006mp}.}\\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 08A & \cite{Noaki:2008iy} & 2 & 1.89 & 2.9
&  \parbox{5cm}{Finite-volume corrections estimates through
  \protect\cite{Colangelo:2005gd}. Additional finite-volume effect for fixed topological charge \protect\cite{Aoki:2007ka}.} \\
[3.0ex] \hline \\[-1.0ex]
%
RBC/UKQCD 08 & \cite{Allton:2008pn} & 2 & 2.74 & 4.6 &  \parbox{5cm}{Finite-volume corrections estimates through \protect\cite{Colangelo:2005gd}. Compare with a previous computation with $V=16^3\times 32$ ($L\simeq 1.83$ fm).}\\
[3.0ex] \hline \\[-1.0ex]
%
PACS-CS 08 & \cite{Aoki:2008sm} & 2 & 2.9 &  2.3 & \parbox{5cm}{Finite-volume corrections estimates through \protect\cite{Colangelo:2005gd}. Compare with a previous computation with $V=20^3\times 40$  ($L\simeq 1.8$ fm).}\\
[3.0ex] \hline \\[-1.0ex]
%
HHS 08 & \cite{Hasenfratz:2008ce} & 2 & 1.84,2.77 &  $\epsilon$-regime &  \parbox{5cm}{Topology: not fixed.}\\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 07B & \cite{Fukaya:2007pn} & 2 & 1.78 & $\epsilon$-regime & \parbox{5cm}{Topology: fixed to $\nu=0$.}\\
[3.0ex]
\hline\hline
%
\end{tabular*}
}


\bigskip
\bigskip
\par\noindent
{\bf Renormalization:}\\
{\footnotesize
\begin{tabular*}{\textwidth}[l]{l @{\extracolsep{\fill}} c c l}
&&& \\[-0.1cm]
\hline\hline
&&& \\[-0.3cm]
Collab. & Ref. & $\Nf$ &  Description \\
\hline\hline
&&& \\[-0.1cm]
%
CERN-TOV 07 & \cite{DelDebbio:2006cn} & 2 &  \parbox{6cm}{Non-perturbative}\\
[3.0ex] \hline \\[-1.0ex]
%
ETMC 07,08A & \cite{Blossier:2007vv,Dimopoulos:2008sy} & 2 & Non-perturbative \\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 08A & \cite{Noaki:2008iy} & 2 & Non-perturbative \\
[3.0ex] \hline \\[-1.0ex]
%
RBC/UKQCD 08 & \cite{Allton:2008pn} & 2 & Non-perturbative\\
[3.0ex] \hline \\[-1.0ex]
%
PACS-CS 08 & \cite{Aoki:2008sm} & 2 & One loop\\
[3.0ex] \hline \\[-1.0ex]
%
HHS 08 & \cite{Hasenfratz:2008ce} & 2 & Non-perturbative \\
[3.0ex] \hline \\[-1.0ex]
%
JLQCD/TWQCD 07B & \cite{Fukaya:2007pn} & 2 & Non-perturbative\\
[3.0ex]
\hline\hline
%
\end{tabular*}
}


%----------------------------------------------------------------------------------------------------------%

\clearpage 

==> conclusion.tex <==
\section{Summary of main results\label{sec:conclusion}}

We end this review with a summary of our main results, but we stress
that they should be considered together with the many comments and
observations which accompany their determination. For the quark masses we
obtain
\begin{eqnarray}
m_s^\msbar(2\,\gev)\al=\al 95\pm 10\,\mev\co \nonumber\\
m_{ud}^\msbar(2\,\gev)\al= \al 3.4\pm0.4\,\mev\co \\
\frac{m_s}{m_{ud}}\al =\al 27.8\pm 1.0\nonumber\co
\end{eqnarray}
where $m_{ud}$ is the average of $m_u$ and $m_d$ and the estimate is based
on $\Nf=2+1$ calculations. These estimates agree with the only $\Nf=2$
determination which satisfies our quality criteria~\cite{Blossier:2007vv}:
\begin{eqnarray}
m_s \al=\al 105 \pm 3 \pm 9 \,\mbox{MeV}\co  \nonumber\\
m_{ud} \al=\al 3.85 \pm 0.12 \pm 0.40  \,\mbox{MeV}  \co  \\
\frac{m_s}{m_{ud}} \al=\al 27.33 \pm 1.2 \co \nonumber
\end{eqnarray}
where the first error is statistical and the second systematic.
The lattice simulations
are performed with $m_u=m_d$, so some additional input is required to
obtain $m_u$ and $m_d$ separately (see the discussion in section
\ref{subsec:mumd}). We quote
\begin{eqnarray}
m_u^\msbar(2\,\gev)\al=\al 2.2\pm0.3\,\mev\co\nonumber\\
m_d^\msbar(2\,\gev)\al=\al 4.6\pm0.6\,\mev\co\\
\frac{m_u}{m_d}\al=\al 0.47\pm 0.04\fs\nonumber
\end{eqnarray}

In the determination of the CKM matrix elements $V_{us}$ and $V_{ud}$, the
term $f_+(0)$ (form factor relevant for the semileptonic transition
$K^0\to\pi^-$, evaluated at zero momentum transfer) and the ratio
$f_K/f_\pi$ of the kaon and pion decay constants play a central role. On
the lattice, both of these quantities can now be determined rather
precisely (we refer to these results, which do not rely on the Standard
Model as {\it direct} determinations, see section \ref{sec:Direct}):
\bea \Nf=2+1, \hspace{0.2cm}\mbox{direct}:\hspace{0.3cm} f_+(0)\al=\al
0.959 \pm 0.005 \,,\hspace{0.5cm}f_K/f_\pi =1.193 \pm 0.006 \,, \\ 
 \Nf=2,\hspace{0.2cm}\mbox{direct}:\hspace{0.95cm} f_+(0)\al=\al
 0.956 \pm 0.008\,,\hspace{0.5cm}f_K/f_\pi =1.210 \pm 0.018 \,. \nonumber
\eea 
 
Two precise experimental results constrain the determination of $V_{us}$
and $V_{ud}$: the observed rate for the semileptonic $K^0\to\pi^-$ decay
determines the product $|V_{us}|f_+(0)$, while the ratios of the kaon's and
pion's leptonic widths determine the ratio $|V_{us}|f_K/|V_{ud}|f_\pi$. In
section \ref{sec:testing}, these results are combined with the lattice
determinations of $f_K/f_\pi$ and $f_+(0)$ to test the unitarity of the CKM
matrix. We find that the first row obeys this property within errors:
$|V_{ud}|^2+|V_{us}|^2+|V_{ub}|^2=1.002(16)$ and $1.036(37)$ for $\Nf =
2+1$ and $\Nf=2$, respectively.\footnote{The experimental information on
  $|V_{ub}|$ shows that the contribution from this term is negligibly
  small.} In obtaining these results, we have not made use of the recent
determinations of $|V_{ud}|$ from super-allowed nuclear
$\beta$-decays. These are perfectly consistent with the outcome of the
lattice calculations. In fact, the unitarity test sharpens considerably if
the results obtained on the lattice are combined with those found in
$\beta$-decay: the range allowed for the sum
$|V_{ud}|^2+|V_{us}|^2+|V_{ub}|^2$ then shrinks by more than an order of
magnitude. Since the range includes unity, CKM unitarity passes the test.

Within the Standard Model of particle physics, the CKM matrix is
unitary. As explained in section \ref{sec:SM}, this condition and the
experimental results for $|V_{us}|f_+(0)$, $|V_{us}|f_K/|V_{ud}|f_\pi$ and
$|V_{ub}|$ imply three equations for the four quantities $|V_{ud}|$,
$|V_{us}|$, $f_K/f_\pi$ and $f_+(0)$. Thus it is sufficient to add one
additional constraint, such as the lattice determination of $f_K/f_\pi$ or
$f_+(0)$, to determine all four of these quantities. Averaging over the
lattice results with $\Nf=2+1$ dynamical quark flavours, we find 
\begin{eqnarray}
|V_{ud}|\al=\al 0.97427 \pm 0.00023 \,, \qquad |V_{us}|=0.2253\pm 0.0010 \,,
\nonumber \\
f_+(0) \al=\al 0.9598 \pm 0.0041 \,, \,\,\,\, \qquad \frac{f_K}{f_\pi}= 1.1924 \pm 0.0054 \,.
\end{eqnarray} 
The results obtained from the data with $\Nf =2$ are the same within errors:
\begin{eqnarray}
|V_{ud}|\al=\al 0.97433 \pm 0.0042 \,, \qquad |V_{us}|=0.2251 \pm 0.0018 \,,
\nonumber \\
f_+(0) \al=\al 0.9604 \pm 0.0075 \,, \, \qquad \frac{f_K}{f_\pi}= 1.194 \pm 0.010 \,.
\end{eqnarray}

As far as the low-energy constants are concerned, there are many results
coming from lattice calculations which are of interest. Not in all cases a
coherent picture emerges yet, but for two quantities related to the SU(2)
chiral expansion the lattice provides results which are competitive with
what has been obtained from the phenomenology. These are
\begin{equation}
\lbar_3 = 3.3 \pm 0.7 \qquad \mbox{and} \qquad \frac{F_\pi}{F}= 1.073 \pm 0.015
\end{equation}
which are estimates based on $\Nf =2$, $\Nf =2+1$ and even $\Nf
=2+1+1$ calculations. We refer the interested reader
to Section~\ref{sec:LECs} for further results and all details about the
calculations.

For the $B_K$ parameter of $K$-$\bar{K}$ mixing we quote:
\begin{equation}
B_K^{\overline{\textrm{MS,NDR}}}(2 \mathrm{GeV})=0.527 \pm0.006 \pm 0.021
\quad\textrm{or equivalently}\quad\hat{B}_K=0.724 \pm 0.008 \pm 0.029 \,
\end{equation}
which is obtained considering only $\Nf=2+1$ results, since no $\Nf=2$
calculation qualifies for entering averages.
